DarTwin made precise by SysMLv2 -- An Experiment

The new SysMLv2 adds mechanisms for the built-in specification of domain-specific concepts and language extensions. This feature promises to facilitate the creation of Domain-Specific Languages (DSLs) and interfacing with existing system descriptions and technical designs. In this paper, we review these features and evaluate SysMLv2's capabilities using concrete use cases. We develop DarTwin DSL, a DSL that formalizes the existing DarTwin notation for Digital Twin (DT) evolution, through SysMLv2, thereby supposedly enabling the wide application of DarTwin's evolution templates using any SysMLv2 tool. We demonstrate DarTwin DSL, but also point out limitations in the currently available tooling of SysMLv2 in terms of graphical notation capabilities. This work contributes to the growing field of Model-Driven Engineering (MDE) for DTs and combines it with the release of SysMLv2, thus integrating a systematic approach with DT evolution management in systems engineering.

==> figures/schematics/NewOutputBefore.tex <==
\begin{tikzpicture}
\node[goal] (goal1) {\textbf{Goal1}}; 

\begin{scope}[yshift=-2.25cm]
    % DT1
    \node[digitaltwin,minimum width=2cm] (dt1) {DT1};

    \node[port,label={below:{}},xshift=-1em] (dt1-in) at (dt1.south) {$\uparrow$};
    \node[port,label={below:{}},xshift=1em] (dt1-out) at (dt1.south) {$\downarrow$};

    \node[port,
        label={[portlabel]below:{}},
        below=.5 of dt1-in,
        ] (outer-in) {$\uparrow$};
    \node[port,
        label={[portlabel]below:{}},
        below=.5 of dt1-out
        ] (outer-out) {$\downarrow$};

    \draw[flow] (outer-in.north) -- (dt1-in.south);
    \draw[flow] (dt1-out.south) -- (outer-out.north);

    % outer system
    \begin{scope}[on behind layer]
       \node[dtsystem,
            label={[below]north:{\textbf{twin system} \emph{name}}},
            fit={(outer-in.east)($(dt1.west)-(2em,0)$)($(dt1.north east)+(2em,1.5em)$)}] (system) {};
    \end{scope}
    
\end{scope}

% relations
\draw[relationToGoal] (dt1) -- (goal1);

\pic (fg-frame) {dartwinFrameFit={New Output/Basic/(goal1)(system)(outer-in)}};
\pic {frameSeparation={fg-frame-box/goal1}};
\end{tikzpicture}
